Temporal Graph Benchmark for Machine Learning on Temporal Graphs

We present the Temporal Graph Benchmark (TGB), a collection of challenging and diverse benchmark datasets for realistic, reproducible, and robust evaluation of machine learning models on temporal graphs. TGB datasets are of large scale, spanning years in duration, incorporate both node and edge-level prediction tasks and cover a diverse set of domains including social, trade, transaction, and transportation networks. For both tasks, we design evaluation protocols based on realistic use-cases. We extensively benchmark each dataset and find that the performance of common models can vary drastically across datasets. In addition, on dynamic node property prediction tasks, we show that simple methods often achieve superior performance compared to existing temporal graph models. We believe that these findings open up opportunities for future research on temporal graphs. Finally, TGB provides an automated machine learning pipeline for reproducible and accessible temporal graph research, including data loading, experiment setup and performance evaluation. TGB will be maintained and updated on a regular basis and welcomes community feedback. TGB datasets, data loaders, example codes, evaluation setup, and leaderboards are publicly available at https://tgb.complexdatalab.com/.

==> 030preliminaries.tex <==
\section{Temporal Graph Notations}
%defining temporal graph
% \subsection{Temporal Graph Notations}

We denote temporal graphs as timestamped edge streams consisting of triplets of source, destination, timestamp; i.e., $\mathcal{G}=\{ (s_0,d_0,t_0), (s_1,d_1,t_1), \dots , (s_T,d_T,T) \} $, where the timestamps are ordered (\textit{$0 \leq t_1 \leq t_2 \leq ... \leq T $})~\cite{poursafaeitowards,kazemi2020representation}. Note that the graph can be directed or undirected, and weighted or unweighted. $\mathcal{G}_t$ is the cumulative graph constructed from all edges in the stream until time $t$ with nodes $\mat{V}_t$ and edges $\mat{E}_t$. Optionally, there can be node features $\mat{X}_t \in \mathbb{R}^{|\mat{V}_t| \times k_x}$, where $k_x$ is the size of the node feature vector, and edge features $\mat{M}_t \in \mathbb{R}^{|\mat{E}_t| \times k_m}$, where $k_m$ is the size of the edge feature vector. We consider a fixed chronological split to form the training, validation and test set. 



\textbf{Evaluation Settings.} There are distinct evaluation settings in temporal graph based on the what test set information is available. We categorize and discuss these setting in detail in Appendix~\ref{app:eval}. In this work, we only consider the \emph{streaming setting} where information from the test set is available only for updating the memory module in various temporal graph learning methods such as TGN~\cite{rossi2020temporal}. However, no weight updates through back-propagation is allowed on the model at test time. 



